Bayesian Pose Graph Optimization via Bingham Distributions and Tempered Geodesic MCMC

We introduce Tempered Geodesic Markov Chain Monte Carlo (TG-MCMC) algorithm for initializing pose graph optimization problems, arising in various scenarios such as SFM (structure from motion) or SLAM (simultaneous localization and mapping). TG-MCMC is first of its kind as it unites asymptotically global non-convex optimization on the spherical manifold of quaternions with posterior sampling, in order to provide both reliable initial poses and uncertainty estimates that are informative about the quality of individual solutions. We devise rigorous theoretical convergence guarantees for our method and extensively evaluate it on synthetic and real benchmark datasets. Besides its elegance in formulation and theory, we show that our method is robust to missing data, noise and the estimated uncertainties capture intuitive properties of the data.

==> change_of_variables.tex <==
\subsection{Change of Variables}
\label{sec:cov}
Lev $V$ and $W$ be bound

==> method.tex <==
%!TEX root = ./bingham_nips2018.tex

\section{3D Pose Representations}
\label{sec:pose}
Any three-dimensional rotation $\mathbf{R}$
is an element of the Special Orthogonal Group $SO(3)$ and satisfies the constraint $\mathbf{R}\mathbf{R}^T = \mathbf{I}$. The exponential and
logarithmic mappings are given by the familiar Rodrigues formula~\cite{}. In turn Euclidean motions, $\mathbf{M} \in SE(3)$ are represented by $4 \times 4$ matrices:
\begin{equation}
\mathbf{M} = 
\begin{bmatrix}
\mathbf{R} & \mathbf{t} \\
\mathbf{0} & 1
\end{bmatrix}
\end{equation}
where $\mathbf{R} \in SO(3)$ and $\mathbf{t} \in \mathbb{R}^3$ are the three-dimensional
rotation and translation respectively. Any point $\mathbf{x} \in \mathbb{R}^3$ transforms (rotates and translates) with the group action:
\begin{equation}
\label{eq:trans}
\mathbf{x}' = \mathbf{M}_{\text{34}}
\begin{bmatrix} \mathbf{x} \\ 1 \end{bmatrix}
=
\mathbf{R}\mathbf{x}+\mathbf{t}
\end{equation}
with $\mathbf{M}_{\text{34}}$ denoting the first 3 rows of $\mathbf{M}$.

\input{quaternions.tex}
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\columnwidth, clip=true]{figures/config01_cropped.pdf}
\caption{Two-camera configuration and the relative pose.}
\label{fig:pose}
\end{figure}
\input{quaternions-se3.tex}

\section{The Multiple Pose Averaging Problem}
\label{sec:averaging}
Let us consider a finite simple directed graph $G = (V, E)$, where vertices correspond to reference frames and edges to the available relative measurements. Both vertices and edges are labeled with rigid motions representing absolute and relative orientations, respectively. Each absolute
orientation is described by a homogeneous transformation matrix $\mathbf{M}_i$ as described in Section \ref{sec:pose}. Similarly, each relative orientation is expressed as $\mathbf{M}_{ij}$, the transformation between frames $i$ and $j$.

The labeling of the edges is such that if $(i, j) \in E$, then $(j, i) \in E$ and $\mathbf{M}_{ij}=\mathbf{M}_{ji}^{-1}$. Hence, we consider $G$ to be undirected. The link between absolute and relative orientations is encoded by the \emph{compatibility constraint}:
\begin{equation}
\mathbf{M}_{ij} = \mathbf{M}_{i}\mathbf{M}_{j}^{-1},\, \forall i \neq j
\end{equation}

The \emph{rigid-motion synchronization problem} requires computing an estimate of the vertex labels
$\mathbf{M}_i$ (absolute poses) given enough measurements of the ratios $\mathbf{M}_j\mathbf{M}_i^{-1}$.

In other words, motion synchronization or multiple motion averaging refers to the problem of recovering absolute motion (poses) of $N$ cameras, from a set of maximum $\frac{N^2-N}{2}$ (fully connected $G$), minimum $N-1$ ($G$ is a tree) relative poses. Typically one of the poses is set to identity $\mathbf{M}_0=\mathbf{I}$ and the problem reduces to recovering $N-1$ absolute orientations

\section{Bingham Distribution}
Let $S^{d-1} = \{\mathbf{x} \in \mathbb{R}^d : \lVert \mathbf{x} \rVert = 1\} \subset R^d$ denote the unit hypersphere in $\mathbb{R}^d$. The Bingham distribution is an antipodally symmetric probability distribution on $S^{d-1}$ with probability density function (PDF) $f : S^{d-1} \rightarrow R$:
\begin{align}
f(\mathbf{x}, \mathbf{\Lambda}, \mathbf{V}) & = \frac{1}{F} \exp(\mathbf{x}^T\mathbf{V}\mathbf{\Lambda}\mathbf{V}^T\mathbf{x}) \\
&= \frac{1}{F} \exp\big(\sum\limits_{i=1}^d \lambda_i(\mathbf{v}_i^T \mathbf{x})^2 \big)
\end{align}
where $\mathbf{V} \in \mathbb{R}^{d\times d}$ is an orthogonal matrix $(\mathbf{V}\mathbf{V}^T = \mathbf{V}^T\mathbf{V} = \mathbf{I}_{d\times d})$ describing the orientation, $\Lambda = diag(\lambda_1, \cdots, \lambda_{d−1}, 0) \in R^{d\times d}$ with $\lambda_1 ≤ \cdots ≤ \lambda_{d-1} \leq 0$ is the inverse covariance (concentration) matrix, and $F$ is a normalization constant.

The pdf is antipodally symmetric, i. e., $f(\mathbf{x}) = f(-\mathbf{x})$ holds for all $\mathbf{x} \in S^{d-1}$.
\paragraph{The Mode} Bingham showed that adding a multiple of the identity matrix $\mathbf{I}_{d\times d}$ to $\mathbf{V}$ does not change the distribution \cite{Bingham1974}. Thus, we conveniently force the last entry of $\mathbf{V}$ to be zero. Moreover, because it is possible to swap columns of $\mathbf{\Lambda}$, we can build $\mathbf{V}$ in a sorted fashion. This allows us to obtain the mode very easily by taking the first column of $\mathbf{V}$. 
\paragraph{The Covariance} 
The covariance matrix $\mathbf{C} \in \mathbf{R}^{d\times d}$ of the Bingham distribution is given by:
\begin{equation}
\mathbf{C} = Cov(\mathbf{x}) = - 0.5(\mathbf{V}(\bm{\Lambda}+c\mathbf{I})\mathbf{V}^T)^{-1}
\end{equation}
where $c \in \mathbb{R}$ can be arbitrarily chosen as long as $(\bm{\Lambda} + c\mathbf{I})$ is negative definite.
%\insertimageC{1}{illustrations_cropped.pdf}{\textbf{(a)}}{fig:visuals}{t!}
\begin{figure}[t!]
\centering
\subfigure[]{
\includegraphics[width=0.57\columnwidth, clip=true]{figures/cameraposes_01.jpg}
}
\subfigure[]{
\includegraphics[width=0.35\columnwidth, clip=true]{figures/binghamPlot.pdf}
}
%\vspace{-1.5em}
\caption{(a) Camera Pose Graph. (b) Bingham distribution when $\mathbf{\lambda}=[-1,-1,-1]^T$ and $F=10$.}
%\vspace{-0.5em}
\label{fig:pose}
\end{figure}


\section{Probabilistic Multiview Pose Synchronization}

\subsubsection*{Cost Function}
\label{sec:cost}\noindent


\subsubsection*{Maximum Likelihood Estimation}
\label{sec:MLE}\noindent
Representing the $SE(3)$ in the form of a quaternion-translation parameterization, the motion-synchronization problem can be solved via the following optimization procedure:
\begin{align}
\label{eq:MLE}
(\mathbf{Q}^*,\mathbf{T}^*) = \argmax_{\mathbf{Q},\mathbf{T}} \Bigg( \sum\limits_i \sum\limits_j \big\{\log p(\mathbf{q}_{ij} | \mathbf{q}_{i}, \mathbf{q}_{j}) \\+ \log p(\mathbf{t}_{ij} | \mathbf{q}_i, \mathbf{q}_j, \mathbf{t}_i, \mathbf{t}_j) \big\}\\ + \sum\limits_i \log p(\mathbf{q}_i) + \sum\limits_i \log p(\mathbf{t}_i) \Bigg)
\end{align}
where $p(\cdot)$ will be modeled using Bingham distributions~\cite{Bingham1974} for quaternions and Gaussian for translations.

\subsubsection*{Probabilistic Multiple Rotation Averaging}
\label{sec:ProbRotations}\noindent
\begin{equation}
\argmax_{\mathbf{q}_{ij}} p(\mathbf{q}_{ij} | \mathbf{q}_{i}, \mathbf{q}_{j}) = \mathbf{q}_{i}\mathbf{q}_{j}^{-1}
\end{equation}

\subsubsection*{Modeling Pose Distributions}
\label{sec:MLE}\noindent
An absolute pose is modeled by the following distributions:
\begin{align}
\mathbf{q}_i \sim \mathcal{B}(\mathbf{\Lambda},\, \mathbf{V})\\
\mathbf{t}_i \sim \mathcal{N}(0,\, \sigma^2 \mathbf{I})
\end{align}
whereas the relative pose obeys:
\begin{align}\label{eq:qijB}
\mathbf{q}_{ij} \, | \, \mathbf{Q} \sim \mathcal{B}(\mathbf{q}_i\mathbf{q}_j^{-1} | \mathbf{\Lambda},\mathbf{V})\\
\mathbf{t}_{ij} \, | \, \mathbf{Q},\mathbf{T} \sim \mathcal{N}(\mathbf{q}_i,\mathbf{q}_j,\mathbf{t}_i,\mathbf{t}_j)
\end{align}

\input{gradients.tex}

\subsubsection{Constructing $\mathbf{V}(\mathbf{r})$}

\subsubsection*{Bingham Quaternions}
\label{sec:BinghamQuat}\noindent
The Bingham distribution with $d = 4$ is used to describe the uncertainty in the space of the unit-quaternions. Our goal is to construct a Bingham distribution with a given mode $\mathbf{q}_{ij}$. As the mode is given by orthogonalization (last column of $\mathbf{V}$, we are required to form $\mathbf{V}$ via the orthogonal vectors.
Constructing Bingham distributions in such a way requires specifying $\mathbf{\Lambda}$ and $\mathbf{V}$, where the former can be set to constant values. Given a unit quaternion $\mathbf{r}$, we can form the columns of $\mathbf{V}=[\mathbf{v}_2, \mathbf{v}_3, \mathbf{v}_4]$ from two means of orthogonalizatinos:
\paragraph{Gram-Schmidt Process}
One way to achieve orthogonalization in N-dimensions is the Gram-Schmidt process. We set the first vector to $\mathbf{v}_1=\mathbf{r}$ and perform the recursion:
%Let $=\mathbf{q}_i\mathbf{q}_j^{-1}
\begin{align}
\mathbf{v}_1 &= \mathbf{r}\label{eq:v1}\\
\mathbf{v}_2 &= \frac{\mathbf{e}_1-{v}_{11} \mathbf{v}_1}{\lVert \mathbf{e}_1-{v}_{11} \mathbf{v}_1 \rVert}\label{eq:v2}\\
\mathbf{v}_3 &= \frac{\mathbf{e}_2 + \mathbf{v}_1({v}_{22}{v}_{11}-{v}_{12})-{v}_{22} \mathbf{e}_1}{\lVert \mathbf{e}_2 + \mathbf{v}_1({v}_{22}{v}_{11}-{v}_{12})-{v}_{22} \mathbf{e}_1 \rVert}\label{eq:v3}\\
\mathbf{v}_4 &= \frac{\mathbf{e}_3 - v_{13}\mathbf{v}_1 - v_{23}\mathbf{v}_2 - v_{33}\mathbf{v}_3}{\lVert \mathbf{e}_3 - v_{13}\mathbf{v}_1 - v_{23}\mathbf{v}_2 - v_{33}\mathbf{v}_3 \rVert}\label{eq:v4}
\end{align}
$\{\mathbf{e}_1 \cdots \mathbf{e}_3\} \in \mathbb{R}^4$ are the unit basis vectors and ${v}_{ij}$  refers to the $j^{th}$ element of vector $i$. Note that this procedure is copmlex, non-linear and computationally expensive to differentiate.
GS process causes $\nabla_{\mathbf{r}}(\mathbf{K}) \in \mathbb{R}^{4 \times 4}$ to take a complex form due to the non-linearities involved. Therefore, it might be a simpler and more sound approach to rely on the algebra of quaternions $\mathbb{H}$ as explained below.

% v4 = e3 - v1(3).*v1 - v2(3).*v2 - v3(3).*v3; v4 = v4./norm(v4);
\paragraph{Parallelizable Manifolds} 
Quaternions lie on the $d-1$ sphere $\mathbf{q} \in S^{d-1}$. A map from the sphere to the frame in the tangent bundle $S^{d-1}\rightarrow FS^{d-1}$ exists for \textit{parallelizable manifolds}. Such frame bundle is composed of the unit vector and its orthonormals. Being parallelizable ($d=1,2,4 \text{ or } 8$), unit quaternions enjoy the following injective homomorphism to the orthonormal matrix ring composed of the orthonormal basis\cite{Steenrod1951}:
%For $d=1,2,4 \text{ and } 8$ the 
\begin{equation}\label{eq:parallel}
\mathbf{q}^T=
\begin{bmatrix}
{q}_1 \\ {q}_2  \\ {q}_3 \\ {q}_4
\end{bmatrix}
\,\rightarrow\,
\mathbf{V}(\mathbf{q})=
\begin{bmatrix}
q_1 & -{q}_2 & -{q}_3 & -{q}_4 \\
q_2 & {q}_1 & {q}_4 & -{q}_3 \\
q_3 & -{q}_4 & {q}_1  & {q}_2 \\
q_4 & {q}_3 & -{q}_2  & {q}_1
\end{bmatrix}
\end{equation}
with $[\mathbf{v}_1 \mathbf{v}_2, \mathbf{v}_3, \mathbf{v}_4]$ referring to columns of $\mathbf{V}(\mathbf{q})$ with $\mathbf{v}_1 = \textbf{q}$.
This is similar to the 2D analogous, where taking the orthonormal is a simple map: $(x,y)\rightarrow (-y, x)$. 

With this definition of $\mathbf{V}(\mathbf{q})$, the terms simplify:
\begin{align}
\mathbf{k}&=
\begin{bmatrix}
q_1 x_1 + q_2 x_2 + q_3 x_3 + q_4 x_4 \\
q_1 x_2 - q_2 x_1 + q_3 x_4 - q_4 x_3 \\
q_1 x_3 - q_3 x_1 - q_2 x_4 + q_4 x_2 \\
q_1 x_4 + q_2 x_3 - q_3 x_2 - q_4 x_1 \\
\end{bmatrix}\\
\nabla_\mathbf{q}(\mathbf{k})&=
\begin{bmatrix}
x_2 & -x_1 & x_4 & -x_3\\
x_3 & -x_4 & -x_1 & x_2\\
x_4 & x_3 & -x_2 & -x_1
\end{bmatrix}
\end{align}

\section{Geodesic MCMC}
\label{GMCMC}
\paragraph{Projection Operator}
As derived in Liu et. al. \cite{Liu2016} (suppl. material A.3), a point $\mathbf{x} \in \mathbb{R}^d$ gets projected \underline{onto the tangent space} $T_x(\Xi(M))$ of a $(d-1)$ dimensional embedded manifold, the hypersphere $S^{d-1}\triangleq \{\mathbf{x} \in \mathbb{R}^d \,|\, \| \mathbf{x} \| = 1\}$, via the following Householder matrix:
\begin{equation}
\mathbf{\Lambda}(\mathbf{x}) = \mathbf{I}_d - \mathbf{x}\mathbf{x}^T
\end{equation}
For a quaternion $\mathbf{q}$ living on the hemisphere, the map for the projection onto the tangent space of the embedded manifold then reads:
\begin{align}
\mathbf{q} &\rightarrow \mathbf{\Lambda}(\mathbf{q})\mathbf{q}\\
&\rightarrow \mathbf{q} - \mathbf{q}\mathbf{q}^T\mathbf{q} = \mathbf{q} - (\mathbf{q} \cdot \mathbf{q})\mathbf{q}
\end{align}
well aligning with the Projection operator implemented at lines 79-81 of GMC.hpp.
\paragraph{High dimensional spheres}
\begin{lemma}
\label{lemma:lambda}
Let $\Phi : \mathbb{R}^d \rightarrow \mathbb{R}^{d \times k} : \{\{\mathbf{q}_i \in \mathbb{R}^d \} \rightarrow \mathbf{x}_i \in \mathbb{R}^{d \times k}, i=1..k\}$ be the \textit{concatenation map}, lifting any $d$-dimensional $k$ points to a $(d \times k)$-dimensional single point. Then if $\{\mathbf{q}_i\} \in \mathbb{R}^d$ lie on the unit sphere $S^{d-1}$, then the point $\mathbf{x}_i$ lies on the high dimensional sphere $S^{d\times k-1}$ of radius $\sqrt{k}$.
\end{lemma}
\begin{proof}
A sphere in $(d \times k)$ dimensional space, $S^{d\times k-1}$ satisfies:
\begin{align}
\sum\limits_{j=1}^{d \times k} x_j^2 = \sum\limits_{j=1}^{d} x_j^2 + \sum\limits_{j=d+1}^{2d} x_j^2 + \cdots + \sum\limits_{j=(k-1)\times d+1}^{d \times k} x_j^2 = r^2
\end{align}
where $\mathbf{x} \in \mathbb{R}^{d \times k}$ and $r$ denotes the radius. 
By definition, each $d$-dimensional subspace of $\mathbb{R}^{d \times k}$ comes from the same unit sphere, i.e. $\mathbf{q}_i = \mathbf{x}_{i d+1:i d +d} \in S^{d-1} : \lVert \mathbf{x}_{i d+1:i d +d} \rVert = 1$:
\begin{align}
\forall i,0\leq i \leq k-1\\
\sum\limits_{i=0}^{k-1} \sum\limits_{j=i d+1}^{i d +d} (x_j)^2 &= r^2 \\
k\sum\limits_{j=i d+1}^{i d +d} (x_j)^2 &=r^2 \\
k \cdot 1 =r^2 \\
r=\sqrt{k}
\end{align}
This suggest that if we add up the unit spheres, we arrive at the high-dimensional sphere $r=\sqrt{k}$. Thus, spaces composed of concatenation of coordinates preserve the spherical manifold structures, only causing a change in the scale. For mapping to the unit sphere in $\mathbb{R}^{dxk}$, one simply applies $\mathbf{x} \rightarrow {\mathbf{x}}/{\sqrt{k}}$.
\end{proof}

==> preamble1.tex <==

%\usepackage[small,compact]{titlesec}

%\usepackage{ulem}

\textheight 9.3in \advance \topmargin by -1.0in \textwidth 6.7in
\advance \oddsidemargin by -0.8in
\newcommand{\myparskip}{3pt}
\parskip \myparskip



%\newenvironment{proofof}[1]{\noindent{\bf Proof of #1.}}%
 %       {\hspace*{\fill}$\Box$\par\vspace{4mm}}

%\documentstyle[12pt,fullpage,graphics,colordvi,amssymb,amsmath,amsthm,eepic]{report}


\newcommand{\tk}{\tilde k}

%\newcommand{\prob}[1]{\ensuremath{\text{{\bf Pr}$\left[#1\right]$}}}
%\newcommand{\expct}[1]{\ensuremath{\text{{\bf E}$\left[#1\right]$}}}
%\newcommand{\expect}[1]{\ensuremath{\text{{\bf E}$[#1]$}}}
%\newcommand{\MSTop}{\operatorname{MST}}
%\newcommand{\MST}{\ensuremath{\MSTop}\xspace}

\newcommand{\connect}{\leadsto}
%\newcommand{\event}{{\cal{E}}}


\newcommand{\dnot}{D^{\circ}}
%--------------------------------------------------------------
%--------------------------------------------------------------
%Problem names
%--------------------------------------------------------------
%--------------------------------------------------------------
\newcommand{\MP}{\mbox{\sf Minimum Planarization}\xspace}
\newcommand{\MCN}{\mbox{\sf Minimum Crossing Number}\xspace}

\newcommand{\MS}{{\sf Machine Scheduling}\xspace}
\newcommand{\RMS}{{\sf Restricted Machine Scheduling}\xspace}
\newcommand{\CM}{{\sf Congestion Minimization}\xspace}
\newcommand{\ST}{{\sf Steiner Tree}\xspace}
\newcommand{\CD}{{\sf Cost-Distance}\xspace}
\newcommand{\PST}{{\sf Priority Steiner Tree}\xspace}
\newcommand{\FCNF}{{\sf FCNF}\xspace}
\newcommand{\AC}{{\sf Asymmetric $k$-Center}\xspace}
\newcommand{\kC}{{\sf $k$-Center}\xspace}
\newcommand{\dH}{{\sf $d$-Hypergraph-Cover}\xspace}
\newcommand{\kH}{{\sf $k$-Hypergraph-Cover}\xspace}
\newcommand{\GS}{{\sf Group-Steiner-Tree}\xspace}
\newcommand{\SC}{{\sf Set-Cover}\xspace}
\newcommand{\GAPSAT}{{\sf Gap-3SAT(5)}\xspace}
\newcommand{\clique}{{\sf Max-Clique}\xspace}
\newcommand{\ML}{{\sf Metric Labeling}\xspace}
\newcommand{\ZE}{{\sf 0-extension}\xspace}
\newcommand{\ZIE}{{\sf $(0,\infty)$-extension}\xspace}
\newcommand{\sat}{{\sf SAT}\xspace}
\newcommand{\mdc}{{\sf MDC}\xspace}
\newcommand{\csp}{{\sf HA-CSP}\xspace}
\newcommand{\NDP}{{\sf NDP}\xspace}
\newcommand{\NDPdisc}{{\sf NDP-Disc}\xspace}
\newcommand{\NDPcyl}{{\sf NDP-Cylinder}\xspace}
\newcommand{\NDPgrid}{{\sf NDP-Grid}\xspace}
\newcommand{\NDPplanar}{{\sf NDP-Planar}\xspace}
\newcommand{\NDPwC}{{\sf NDPwC}\xspace}
\newcommand{\EDPwC}{{\sf EDPwC}\xspace}

\newcommand{\EDP}{{\sf EDP}\xspace}

\newcommand{\DPSP}{{\sf DPSP}\xspace}

\newcommand{\yi}{{\sc Yes-Instance}\xspace}
\renewcommand{\ni}{{\sc No-Instance}\xspace}
\newcommand{\Gr}[1]{G^{(#1)}}
\newcommand{\Hr}[1]{H^{(#1)}}


\newcommand{\optmp}[1]{\mathsf{OPT}_{\mathsf{MP}}(#1)}
\newcommand{\optcro}[1]{\mathsf{OPT}_{\mathsf{cr}}(#1)}
%\newcommand{\optcro}[1]{\mathsf{OPT}_{\mathsf{cr}}(#1)}
\newcommand{\optcre}[1]{\mathsf{OPT}_{\mathsf{cre}}(#1)}

\newcommand{\optcrosq}[1]{\mathsf{OPT}^{2}_{\mathsf{cr}}(#1)}
\newcommand{\algsc}{\ensuremath{{\mathcal{A}}_{\mbox{\textup{\footnotesize{AKR}}}}}\xspace}
\newcommand{\alphasc}{\ensuremath{\alpha_{\mbox{\textup{\footnotesize{\tiny{AKR}}}}}}}
\newcommand{\dface}{d_{\mbox{\textup{\footnotesize{GNC}}}}}
\newcommand{\tgamma}{\tilde{\gamma}}
%\newcommand{\cro}{\mathsf{cr}}
\newcommand{\bad}{\mathsf{bad}}
%\newcommand{\dmax}{d_{\mbox{max}}}
\newcommand{\G}{{\mathbf{G}}}
\renewcommand{\H}{{\mathbf{H}}}
\newcommand{\bphi}{{\boldsymbol{\varphi}}}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
%--------------------------------------------------------------
%--------------------------------------------------------------
%Protocol names
%--------------------------------------------------------------
%--------------------------------------------------------------
\newcommand{\RP}{{\sc 1R2P}\xspace}
\newcommand{\RV}{{\sc Raz Verifier}\xspace}

%--------------------------------------------------------------
%--------------------------------------------------------------
%Math operators
%--------------------------------------------------------------
%--------------------------------------------------------------
\newcommand{\size}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\Dexp}[1]{\dexp\{#1\}}
\newcommand{\Tower}[2]{\operatorname{tower}^{(#1)}\{#2\}}
\newcommand{\logi}[2]{\operatorname{log}^{(#1)}{#2}}
\newcommand{\norm}[1]{\lVert #1\rVert}
\newcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\paren}[1]{\left ( #1 \right ) }
\newcommand{\union}{\cup}
\newcommand{\band}{\wedge}
\newcommand{\bor}{\vee}

\newcommand{\psd}{\succeq}



\newcommand{\event}{{\cal{E}}}


\newenvironment{propertiesl}[2][1]{
	\begin{enumerate}[label={\normalfont (\ref{#2}\alph*)},labelwidth=*,leftmargin=*,itemsep=0pt,topsep=3pt, start=#1]
}{
	\end{enumerate}
}
%--------------------------------------------------------------
%--------------------------------------------------------------
%Complexity Classes
%--------------------------------------------------------------
%--------------------------------------------------------------

\renewcommand{\P}{\mbox{\sf P}}
\newcommand{\NP}{\mbox{\sf NP}}
\newcommand{\PCP}{\mbox{\sf PCP}}
\newcommand{\ZPP}{\mbox{\sf ZPP}}
\newcommand{\polylog}[1]{\mathrm{polylog(#1)}}
\newcommand{\DTIME}{\mbox{\sf DTIME}}
\newcommand{\ZPTIME}{\mbox{\sf ZPTIME}}

\newcommand{\opt}{\mathsf{OPT}}

\newcommand{\alphawl}{\ensuremath{\alpha_{\mbox{\tiny{\sc WL}}}}}
\newcommand{\alphaWL}{\ensuremath{\alpha_{\mbox{\tiny{\sc WL}}}}}


%--------------------------------------------------------------
%--------------------------------------------------------------
%Sets
%--------------------------------------------------------------
%--------------------------------------------------------------
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\sse}{\subseteq}


%General Environments
%--------------------------------------------------------------
%--------------------------------------------------------------

\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}


%--------------------------------------------------------------
%--------------------------------------------------------------
%Theorems and such
%--------------------------------------------------------------
%--------------------------------------------------------------

\def\stopproof{\square}
\def\square{\vbox{\hrule height.2pt\hbox{\vrule width.2pt height5pt \kern5pt
\vrule width.2pt} \hrule height.2pt}}


\newcommand{\tw}{\mathrm{tw}}

%--------------------------------------------------------------
%--------------------------------------------------------------
%Figures and such
%--------------------------------------------------------------
%--------------------------------------------------------------
\newcommand{\scale}[2]{\scalebox{#1}{#2}}

\newcommand{\fig}[1]{
\begin{figure}[h]
\rotatebox{0}{\includegraphics{#1}}
\end{figure}}

\newcommand{\figcap}[2]
{
\begin{figure}[h]
\rotatebox{270}{\includegraphics{#1}} \caption{#2}
\end{figure}
}

\newcommand{\scalefig}[2]{
\begin{figure}[h]
\scalebox{#1}{\includegraphics{#2}}
\end{figure}}

\newcommand{\scalefigcap}[3]{
\begin{figure}[h]
\scalebox{#1}{\rotatebox{0}{\includegraphics{#2}}} \caption{#3}
\end{figure}}

\newcommand{\scalefigcaplabel}[4]{
\begin{figure}[h]
 \scalebox{#1}{\includegraphics{#2}}\caption{#3\label{#4}}
\end{figure}}

%-----------------------------------------------------
%Programs
%-----------------------------------------------------
%\newenvironment{prog}[1]{
%\begin{minipage}{5.8 in}
%\begin{center}
%{\sc #1}
%\end{center}
%\begin{itemize}}
%{
%\end{itemize}
%\end{minipage}}

\newcommand{\program}[2]{\fbox{\vspace{2mm}\begin{prog}{#1} #2 \end{prog}\vspace{2mm}}}
%-----------------------------------------------------------

%--------------------------------------------------------------
%--------------------------------------------------------------
%Other - Math
%--------------------------------------------------------------
%--------------------------------------------------------------
\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\epsilon}
\newcommand{\Sum}{\displaystyle\sum}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\dist}{\mbox{\sf dist}}

\newcommand{\reals}{{\mathbb R}}
\newcommand{\one}{{\mathbf{1}}}


%first parameter is optional
\newcommand{\expect}[2][]{\text{\bf E}_{#1}\left [#2\right]}
\newcommand{\prob}[2][]{\text{\bf Pr}_{#1}\left [#2\right]}

\newcommand{\four}[1]{\widehat {#1}}
\newcommand{\fourf}{\widehat {f}}
\newcommand{\fourg}{\widehat {g}}
\newcommand{\chisx}{\chi_S(x)}
\newcommand{\chitx}{\chi_T(x)}
\newcommand{\chisy}{\chi_S(y)}
\newcommand{\chity}{\chi_T(y)}
\newcommand{\chiwx}{\chi_W(x)}
\newcommand{\chiwy}{\chi_W(y)}
\newcommand{\chis}{\chi_S}
\newcommand{\chit}{\chi_T}
\newcommand{\chiw}{\chi_W}
\newcommand{\chisminust}{\chi_{S\triangle T}}

%First parameter: index from which counting starts is optional, default is 1; second parameter is the %letter before the property indices
%Example: \begin{properties}{C} or \begin{properties}[5]{C} will start with C6
\newenvironment{properties}[2][0]
{\renewcommand{\theenumi}{#2\arabic{enumi}}
\begin{enumerate} \setcounter{enumi}{#1}}{\end{enumerate}\renewcommand{\theenumi}{\arabic{enumi}}}


\setlength{\parskip}{2mm} \setlength{\parindent}{0mm}

\newcommand{\mynote}[1]{{\sc\bf{[#1]}}}
\newcommand{\fillin}{{\sc \bf{[Fill in]}}}
\renewcommand{\check}{{\sc \bf{[Check!]}}}
\newcommand{\explain}{{\sc \bf{[Explain]}}}


\newcommand{\notsat}[1]{\overline{\text{SAT}(#1)}}
\newcommand{\notsats}[2]{\overline{\text{SAT}_{#1}(#2)}}

\newcommand{\sndp}{\mbox{\sf SNDP}}
\newcommand{\ecsndp}{\mbox{\sf EC-SNDP}}
\newcommand{\vcsndp}{\mbox{\sf VC-SNDP}}
\newcommand{\kec}{k\mbox{\sf -edge connectivity}}
\newcommand{\kvc}{k\mbox{\sf -vertex connectivity}}
\newcommand{\sskec}{\mbox{\sf single-source}~k\mbox{\sf -edge connectivity}}
\newcommand{\sskvc}{\mbox{\sf single-source}~k\mbox{\sf -vertex connectivity}}
\newcommand{\subkvc}{\mbox{\sf subset}~k\mbox{\sf -vertex connectivity}}
\newcommand{\oneec}{1\mbox{\sf -edge connectivity}}
\newcommand{\onevc}{1\mbox{\sf -vertex connectivity}}
\newcommand{\kvcssp}{k\mbox{\sf -vertex-connected spanning subgraph problem}}


\newcommand{\dmax}{d_{\mbox{\textup{\footnotesize{max}}}}}


\newcommand{\face}{\mathrm{face}}
\mathchardef\hyphen="2D
\newcommand{\mincycle}{\mathrm{min\hyphen cycle}}

\newcommand{\out}{\operatorname{out}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\cre}{\operatorname{cre}}
\newcommand{\tC}{\tilde C}


\newcommand{\cclass}[2]{\mathcal{S}_{#1}^{(#2)}}
\newcommand{\tcclass}[2]{\tilde{\mathcal{S}}_{#1}^{(#2)}}

%template for primal-dual
%\begin{tabular}[t]{|l|l|}\hline &\\
%$\begin{array}{lll}
%\text{\underline{Primal}}&&\\
%\text{Max}&\sum_i\sum_{p\in \pset_i}f(p)&\\
%\text{s.t.}&&\\
%&\sum_{p\in\pset_i}f(p)\leq 1&\forall 1\leq i\leq k\\
%\end{array}$
%&$
%\begin{array}{lll}
%\text{\underline{Dual}}&&\\
%\text{Min}&\sum_{i=1}^kz_i+\sum_{e\in E}x_e\\
%\text{s.t.}&&\\
%&z_i+\sum_{e\in p}x_e\geq 1&\forall 1\leq i\leq k, p\in\pset_i\\
%\end{array}$\\ &\\ \hline
%\end{tabular}


%------------------------------------------------------------
%Making subfigures
%------------------------------------------------------------

%\begin{figure}[h]
%\centering
%\subfigure[caption subfigure 1]{\scalebox{0.2}{\includegraphics{file1..pdf}}\label{fig: label1}}
%\hspace{1cm}
%\subfigure[caption subfigure 2]{
%\scalebox{0.2}{\includegraphics{file2.pdf}}\label{fig: label2}}
%\hspace{1cm}
%\subfigure[caption subfigure 3]{\scalebox{0.2}{\includegraphics{file3.pdf}}\label{fig: label3}}
%\caption{caption for the whole figure\label{fig: whole figure}}
%\end{figure}


%------------------------------------------------------------
%Regular figures
%------------------------------------------------------------

%\begin{figure}[h]
% \scalebox{0.3}{\includegraphics{file.pdf}}\caption{CAPTION \label{fig: label}}
%\end{figure}

==> quaternions-se3.tex <==
\subsection{Quaternions and $\text{SE}(3)$}
\label{sec:quatsRelPose}\noindent
Rigid transformation in eq.~\ref{eq:trans} can simply be re-written using the quaternions in a similar manner:
\begin{equation}
\mathbf{x}' = \mathbf{R}\mathbf{x}+\textbf{t}=\mathbf{q}\cdot\mathbf{x}\cdot\bar{\mathbf{q}} + \mathbf{t}
\end{equation}
The $\text{SE}(3)$ parameterization admits the bijective inverse map:
\begin{equation}
\begin{bmatrix} \textbf{q} \\ \mathbf{t} \end{bmatrix} \rightleftarrows
\begin{bmatrix} \bar{\textbf{q}} \\ -\bar{\textbf{q}} \cdot \mathbf{t} \cdot {\textbf{q}} \end{bmatrix}
\end{equation}
The relative pose between two coordinate frames become:
\begin{align}
\mathbf{q}_{i \rightarrow j} &= {\mathbf{q}}_j\cdot\bar{\mathbf{q}}_i\\
\mathbf{t}_{i \rightarrow j} &= \mathbf{t}_j - \bar{\mathbf{q}}_{i \rightarrow j}\cdot\bar{\mathbf{t}}_i\cdot\bar{\mathbf{q}}_{i \rightarrow j}
\end{align}
% = \mathbf{t}_j - \bar{\mathbf{q}}_i\cdot\mathbf{{q}}_j\cdot\bar{\mathbf{t}}_i\cdot\mathbf{\bar{q}}_j\cdot\bar{\mathbf{q}}_i

==> quaternions.tex <==
%%%%%%%%% %%%%%%%%% Quaternions
\subsection{Quaternions}
\label{sec:quaternions}\noindent
Quaternions extend the complex numbers with three imaginary units $\textbf{i}$, $\textbf{j}$, $\textbf{k}$. A \textbf{quaternion} $\q$ is an element of the algebra $\mathbb{H}$ in the form
  \begin{align}
		\q
		= q_1 \textbf{1} + q_2 \textbf{i} + q_3 \textbf{j} + q_4 \textbf{k}
    = \left(q_1, q_2, q_3, q_4\right)^{\text{T}},
	\end{align}
		with $\left(q_1, q_2, q_3, q_4\right)^{\text{T}} \in \mathbb{R}^4$ and
$\textbf{i}^2 = \textbf{j}^2 = \textbf{k}^2 = \textbf{i}\textbf{j}\textbf{k} = - \textbf{1}$.

We also write $\q := \left[a, \textbf{v}\right]$ with the scalar part $a = \q_1 \in \mathbb{R}$ and the vector part $\textbf{v} = \left(q_2, q_3, q_ 4\right)^{\text{T}} \in \mathbb{R}^3$.
The conjugate $\bar{\q}$ of the quaternion $\q$ is given by
\begin{align}
	\bar{\q} := q_1 - q_2 \textbf{i} - q_3 \textbf{j} - q_4 \textbf{k}.
\end{align}
Quaternions are of particular interest in computer vision due to their connection with spatial rotations~\cite{Faugeras2001}.
A versor or \textbf{unit quaternion} $\q \in \mathbb{H}_1$ with $1 \stackrel{\text{!}}{=} \left\|\q\right\|
	:= \q \cdot \bar{\q}$
gives a compact and numerically stable parametrization to represent orientation and rotation of objects in $\mathbb{R}^3$ which avoids gimbal lock~\cite{Lepetit2005}.

\subsubsection*{Quaternion Inverse}
The inverse of quaternion $\q$ has the form:
\begin{equation}
\q^{-1}= {\bar{\q}}/{\lVert \bar{\q} \rVert^2}
\end{equation}
For a unit quaternion, inversion equates to the conjugation.
\subsubsection*{Quaternion Product}
\label{sec:quatsProd}\noindent
The non-commutative multiplication of two quaternions $\mathbf{p}:=[p_1, \mathbf{v}_p]$ and $\mathbf{r}:=[r_1, \mathbf{v}_r]$ is defined to be:
\begin{equation}
\textbf{p}\otimes\textbf{r} =
[{p}_1{r}_1-\mathbf{v}_p\cdot \mathbf{v}_r,\,{p}_1\mathbf{v}_r+{r}_1 \mathbf{v}_p+\mathbf{v}_p \times \mathbf{v}_r]
\end{equation}
For simplicity of notation, we will use $\textbf{p}\otimes\textbf{r}:=\textbf{p}\cdot\textbf{r}:=\textbf{p}\textbf{r}$ for quaternions.
%%%%%%%%% Rotations
\subsubsection*{Rotations with Quaternions}
\label{sec:quatsRot}\noindent
The rotation around the unit axis $\textbf{v} = \left(v_1,v_2,v_3\right)^{\text{T}} \in \mathbb{R}^3$ with angle $\theta$ is thereby given by
\begin{align}
  \textbf{r}= 
  \begin{bmatrix}
  \cos \left( \theta / 2 \right) & \sin \left( \theta / 2 \right) \textbf{v}^T
  \end{bmatrix}^T.
	\label{rotQuat}
\end{align}
Identifying antipodal points $\q$ and $-\q$ with the same element in $SO\left(3\right)$, the unit quaternions form a double covering group of the 3D rotations and any \textbf{point quaternion} or pure quaternion
\begin{align}
	\textbf{p}(\textbf{u})
	= x \textbf{i} + y \textbf{j} + z \textbf{k}
	\label{pointQuat}
\end{align}
of the point $\textbf{u} = \left(x,y,z\right)^{\text{T}} \in \mathbb{R}^ 3$ is rotated by the versor $\textbf{r}$ via the sandwiching product map
\begin{align}
	\textbf{p}
	\mapsto \textbf{r} \cdot \textbf{p} \cdot \bar{\textbf{r}}.
\end{align}
\subsubsection*{Derivatives with Quaternions}
\label{sec:quatsDeriv}\noindent
The rotated quaternion $\mathbf{p}\prime=\mathbf{r}\mathbf{p}\mathbf{\bar{r}}$ needs to be differentiated with respect to the rotating quaternion $\mathbf{r}$, when the rotation is estimated from numerical optimization. The derivative can be represented using the matrix calculus notation:
\begin{align}
&\frac{\partial \mathbf{p}\prime}{\partial \mathbf{r}}=\Bigg[
\frac{\partial \mathbf{p}\prime}{\partial \mathbf{r}_1},
\frac{\partial \mathbf{p}\prime}{\partial \mathbf{r}_2},
\frac{\partial \mathbf{p}\prime}{\partial \mathbf{r}_3},
\frac{\partial \mathbf{p}\prime}{\partial \mathbf{r}_4}
\Bigg]\\
&=[\textbf{p}\q- \overbar{\textbf{pq}}, \overbar{\textbf{pqi}}-\textbf{pqi},
\overbar{\textbf{pqj}}-{\textbf{pqj}},
\overbar{\textbf{pqk}}-\textbf{pqk}]
\end{align}

\subsubsection*{Relative Quaternion Rotation}
\label{sec:quatsRelPose}\noindent
The relative orientation between two quaternions $\q$ and $\mathbf{p}$ is obtained simply by non-commutative Quaternion division:
\begin{equation}
\mathbf{r} = \q\otimes\mathbf{p}^{-1}.
\end{equation}

